Visualizing Streaming Text Data with Dynamic Maps

The many endless rivers of text now available present a serious challenge in the task of gleaning, analyzing and discovering useful information. In this paper, we describe a methodology for visualizing text streams in real time. The approach automatically groups similar messages into "countries," with keyword summaries, using semantic analysis, graph clustering and map generation techniques. It handles the need for visual stability across time by dynamic graph layout and Procrustes projection techniques, enhanced with a novel stable component packing algorithm. The result provides a continuous, succinct view of evolving topics of interest. It can be used in passive mode for overviews and situational awareness, or as an interactive data exploration tool. To make these ideas concrete, we describe their application to an online service called TwitterScope.

==> abs.tex <==
The many endless rivers of text now available present a serious challenge in
the task of gleaning, analyzing and discovering useful information.
In this paper, we describe a methodology for visualizing text streams in
real time. The approach automatically groups similar messages into ``countries,''
with keyword summaries, using semantic analysis, graph clustering and
map generation techniques. It handles the need for visual stability 
across time by dynamic graph layout and Procrustes projection techniques,
enhanced with a novel stable component packing algorithm. The result provides
a continuous, succinct view of evolving topics of interest.
It can be used in passive mode for overviews and situational awareness,
or as an interactive data exploration tool.
To make these ideas concrete, we describe their application 
to an online service called TwitterScope.


==> conc.tex <==
\section{Conclusion\label{sec_conc}}

We presented a general technique for visualizing real-time streams of
text packets. It clusters packets into subtopics based
on semantic analysis and, using a geographic map metaphor, renders
subtopics as countries, with an attached textual precis.
The approach relies on placement algorithms that promote the 
stability of the drawing to aid a user's comprehension,
In particular, we introduced a new packing algorithm to address
component stability.

We see two obvious algorithmic enhancements for our current approach, both
dealing with visual stability. First, when we recreate the map, colors 
for countries are assigned without much consideration to
stability. There has been recent work on achieving color assignment stability
that we would like to incorporate \cite{Hu_Kobourov_Veeramoni_2012_matching}.
Second, for certain topics,
when we perform a periodic packing refresh, the map may change significantly.
It would be good to avoid this discontinuity, either algorithmically or visually.

We would like to deploy TwitterScope as a visual search engine,
allowing arbitrary keyword search instead of the fixed number of topics 
available in the current implementation. This will require a modified system
architecture, including server-side query handling, but we don't envision
any major changes to the algorithms described above.

At present, back-end processes handle most of the data filtering and analysis.
As part of making the system more flexible, we expect to re-implement most
of these processes in JavaScript so
the computing and networking load can be shifted to the client side.
This would mean shifting the clustering, mapping, dynamic layout, 
and component packing to the browser. While this is not easy to implement,
having these algorithms available in clients would open new possibilities
for other sophisticated visualization tasks.


==> related.tex <==
\section{Related Work}

Visualizing streams of text is an active area of research, especially
with the growth of social media and related interest in
gaining insight about this data. %commercializing this data.
\v{S}ili\'{c} \cite{survey_2010} gives a recent survey.
Much of this work has a different focus from ours, dealing with the statistical
analysis and presentation of topics or terms, focusing on the emergence of topic events \cite{Cui_2011_textflow},
and often relying on off-line processing \cite{DBLP:conf/chi/MarcusBBKMM11}.
Our approach focuses on the visualization of the text messages themselves, arriving in real-time.
Topic information emerges from the display of the messages.

For example,
the TextPool visualization proposed by Albrech-Buehler {\em et al.} \cite{textpool_2005} 
scans summaries of new articles,
gathers important terms from the packets, determines connectedness between terms
based on co-occurrence and other measures, and draws the resulting graph. The graph
evolves over time as terms and edges appear and disappear; graph stability is achieved by
using force-directed placement. There is always just one component.

A context-preserving dynamic text
visualization proposed by Cui {\em et al.}~\cite{Cui_2010_wordcloud} displays word clouds
to glean information from a collection of documents over time,
keeping their layout stable using a spring embedding algorithm, aided by
a mesh constructed over existing nodes. 


TopicNets \cite{topicnets_2012} analyzes large text corpora off-line.
The main view is of a document-topic graph, though the system also allows aggregate
nodes. Topic similarity is determined using Latent Dirichlet Allocation (LDA), with topics
then positioned using multidimensional scaling. After topics fixed, documents are
positioned using force-directed placement. 
The time dimension is handled by a separate visualization, with documents placed chronologically
around a (broken) circle, and connected to related topic nodes placed inside the circle.

Alsakran {\em et al.} offer another approach in STREAMIT \cite{streamit_2012}.
This system displays messages or documents positioned using a spring-based force-directed placement, 
where the ideal spring length is based on similarity of keyword vectors of documents. 
Scalability is achieved by 
parallelization on a GPU. Clustering is based on geometry, a second-order attribute, rather than directly on content.
Clusters are labeled with the title of the most recent document joining the cluster.

Our work differs from the above in that we use a map metaphor to visualize clusters.
We do not assume that the underlying content graph is connected.
Our proposal supports monitoring text streams in real time.

In our approach, for semantic analysis, we considered the options of
either LDA, or term frequency-inverse document frequency, to derive message-to-message similarity.
We find clusters directly from this similarity.
Our visualization is focused on the discrete messages as they arrive, and
rather than presenting just items or node-link diagrams, we display messages within a geographic map
metaphor, where topics are depicted as countries. This provides an aid to comprehension \cite{Fabrikant_2006_map_infoviz}.
Edges are still shown to give a sense of connectivity, as there may not be edges between some topic
countries.
These objectives create new problems in maintaining visual stability over time. In the our
approach, beyond the stasis provided by basic graph layout, we apply Procrustes transformation
to documents within a component, and propose a stable packing algorithm for components to achieve further stability.

Focusing on the underlying layout algorithms,
we note the large body of prior research on dynamic graph
layout, in which the goal is to maintain a stable layout of a graph as it is
modified via operations, typically insertion or deletion of nodes and edges.
Brandes and Wagner adapt a force-directed
model to dynamic graphs using a Bayesian framework~\cite{bw-bpdgl-98},
while Herman {\em et al.}~\cite{herman00graph} rely on good static
layouts. Diehl and G{\"o}rg~\cite{Diehl:2002:GTC} consider graphs in
a sequence to create smoother transitions. Brandes and
Corman~\cite{brandes-corman02} present a system for visualizing
network evolution in which each modification is shown in a separate
layer of a 3D representation, with nodes common to two layers
represented as columns connecting the layers. Thus, mental map
preservation is achieved by pre-computing good locations for the nodes
and fixing those positions across the layers. 
Most recently, Brandes and Mader \cite{Brandes_2011_dyn_offline} 
studied offline dynamic graph drawings and compared various
techniques such as aggregation (forming a large graph of all nodes
of all time steps), anchoring (tying nodes to the previous positions) 
and linking (linking nodes from successive time steps, \cite{graphael}), 
and found linking
to be a generally preferred approach, followed by anchoring.
While the issue of
mental map preservation adopted in such approaches remains an
important research issue, we note that in our application we want to avoid
distortion of the layout for the purpose of mental stability. This
is because such distortions introduce biases that can persist over
time. In addition we want a fast procedure suitable for online
dynamic layout. Hence we do not use techniques such as anchoring or
linking, or ones that rely on offline processing of a given sequence
of graphs.

Although there does not appear to have been much previous work on
stably packing complex objects (Section~\ref{sec_packing}), there has
been much work on the related problem of stably removing node overlap ({\it e.g.} \cite{Dwyer_Marriott_Stuckey_2005,Gansner_Hu_2008,Gansner_North_1998}).
This has been limited to removing overlaps of simple shapes, and not aimed at packing them.
On the other hand, there has also been work on optimal unrestricted placement of complex shapes.
Landesberger {\em et al.} \cite{Landesberger_2009_components_cluster} studied ways of clustering
disconnected components for visual analysis.
Freivalds {\em et al.} \cite{Freivalds_2002_polyominos} proposed a polyomino-based algorithm for packing disconnected components.
And Goehlsdorf {\em et al.} \cite{Goehlsdorf_207_disconnected} introduced
new quality measures to evaluate two-dimensional configurations, which yield more compact layouts.


